Influence Function based Data Poisoning Attacks to Top-N Recommender Systems

Recommender system is an essential component of web services to engage users. Popular recommender systems model user preferences and item properties using a large amount of crowdsourced user-item interaction data, e.g., rating scores; then top-$N$ items that match the best with a user's preference are recommended to the user. In this work, we show that an attacker can launch a data poisoning attack to a recommender system to make recommendations as the attacker desires via injecting fake users with carefully crafted user-item interaction data. Specifically, an attacker can trick a recommender system to recommend a target item to as many normal users as possible. We focus on matrix factorization based recommender systems because they have been widely deployed in industry. Given the number of fake users the attacker can inject, we formulate the crafting of rating scores for the fake users as an optimization problem. However, this optimization problem is challenging to solve as it is a non-convex integer programming problem. To address the challenge, we develop several techniques to approximately solve the optimization problem. For instance, we leverage influence function to select a subset of normal users who are influential to the recommendations and solve our formulated optimization problem based on these influential users. Our results show that our attacks are effective and outperform existing methods.

==> macros.tex <==

%
% The name of this file is ``macros.tex''
%

%
% TEX defaults
%
%
% frame 6.5 * 9
\textwidth 6.5in
\textheight 9in

% left/right margins
\oddsidemargin 0pt
\evensidemargin 0pt
\marginparwidth 1in
\marginparsep 0pt

% top margin
\topmargin -25pt
\headheight 10pt
\headsep 30pt
% \topskip 0pt

% foot margin
%\footheight 0pt
\footskip 27pt


% macros for commonly used special fonts
\newcommand{\IE}{{\it i.e.,}\ }
\newcommand{\EG}{{\it e.g.,}\ }
% single/double spacing
%\newcommand{\SS}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\DS}{\renewcommand{\baselinestretch}{1.6}\large\normalsize}
% reduce the space between lines
\newcommand{\Tight}{\renewcommand{\baselinestretch}{0.9}\large\normalsize}
\newcommand{\HalfTight}{\renewcommand{\baselinestretch}{0.95}\large\normalsize}
\newcommand{\MinorTight}{\renewcommand{\baselinestretch}{0.975}\large\normalsize}
% Page title (primarily for foils)
% (this was called \HH}
\newcommand{\PageTitle}[1]{{\newpage \begin{center}{\LARGE {\bf {#1}} } \end{center} } }

% remove spaces around section headers
%\newcommand{\Section}[1]{\vspace{-3ex}\section{#1}\vspace{-2ex}}
\newcommand{\Subsection}[1]{\vspace{-2ex}\subsection{#1}\vspace{-1ex}}
\newcommand{\Subsubsection}[1]{\vspace{-2ex}\subsubsection{#1}\vspace{-1ex}}

% go forward n lines (negative for backward move)
\newcommand{\VLine}[1]{\vspace{#1ex}}
% itemize and enumerate without spaces around/between items
\newenvironment{TightItem}{\vspace{-2ex}\begin{itemize}
  \setlength{\itemsep}{-0ex}}{\end{itemize}\vspace{-1ex}}
\newenvironment{TightEnum}{\vspace{-2ex}\begin{enumerate}
  \setlength{\itemsep}{-0ex}}{\end{enumerate}\vspace{-1ex}}
\newenvironment{TightDesc}{\vspace{-1ex}\begin{description}
  \setlength{\itemsep}{-0ex}}{\end{description}\vspace{-1ex}}
% set the page number (to the first argument)
\newcommand{\SetPageNo}[1]{\countdef\pageno=0 \pageno=#1}
% things to do
\newenvironment{Todo}{\begin{large}\begin{bf}********** things to do
    ********** \\}{\\ **********\end{bf}\end{large}}
% for discussion
\newenvironment{Discuss}{\begin{large}\begin{em}**********
    things to be discussed ********** \\}{\\ **********\end{em}\end{large}}
% set the paragraph identation and separation


% the foil environment
\newenvironment{Foil}{\begin{document}\begin{LARGE}\begin{sf}
    }{\end{sf}\end{LARGE}\end{document}}
    % NOTE: ``}'' must be in the 2nd line
% foil page title
\newcommand{\Title}[1]{\newpage \center{\huge {\sf #1}} \flushleft
    \vspace{1ex}}

% set the paragraph identation and separation
\parindent 0.2in
\setlength{\parskip}{1ex}

% set text width
\textwidth = 6.75in

% set the formula separation
\setlength{\topsep}{0in}

% set indentation for formulas:
% \setlength{\mathindent}{3ex}

% set left margin
\setlength{\oddsidemargin}{-.1in}



